Exposure to Content Written by Large Language Models Can Reduce Stigma Around Opioid Use Disorder in Online Communities

Widespread stigma, both in the offline and online spaces, acts as a barrier to harm reduction efforts in the context of opioid use disorder (OUD). This stigma is prominently directed towards clinically approved medications for addiction treatment (MAT), people with the condition, and the condition itself. Given the potential of artificial intelligence based technologies in promoting health equity, and facilitating empathic conversations, this work examines whether large language models (LLMs) can help abate OUD-related stigma in online communities. To answer this, we conducted a series of pre-registered randomized controlled experiments, where participants read LLM-generated, human-written, or no responses to help seeking OUD-related content in online communities. The experiment was conducted under two setups, i.e., participants read the responses either once (N = 2,141), or repeatedly for 14 days (N = 107). We found that participants reported the least stigmatized attitudes toward MAT after consuming LLM-generated responses under both the setups. This study offers insights into strategies that can foster inclusive online discourse on OUD, e.g., based on our findings LLMs can be used as an education-based intervention to promote positive attitudes and increase people's propensity toward MAT.

==> figures/figure3-raw_change.tex <==
\begin{figure*}
\centering
    \begin{subfigure}[b]{0.33\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/raw_scores_DV1_single-shot.png}
    \caption{} \label{fig:raw_single_DV1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.33\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/raw_scores_DV2_single-shot.png}
    \caption{} \label{fig:raw_single_DV2}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.33\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/raw_scores_DV3_single-shot.png}
    \caption{} \label{fig:raw_single_DV3}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.33\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/raw_scores_DV1_repeated-exp.png}
    \caption{} \label{fig:raw_repeated_DV1}
    \end{subfigure}
    \begin{subfigure}[b]{0.33\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/raw_scores_DV2_repeated-exp.png}
    \caption{} \label{fig:raw_repeated_DV2}
    \end{subfigure}
    \begin{subfigure}[b]{0.33\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/raw_scores_DV3_repeated-exp.png}
    \caption{} \label{fig:raw_repeated_DV3}
    \end{subfigure}
    \caption{\emph{Raw or Actual Change in Participant Attitudes (post-intervention).} \textbf{(a)}, \textbf{(b)}, and \textbf{(c)}: raw change in attitudes (i.e., $\delta Y = Y_{post} - Y_{pre}$) aggregated across participants, after participating in the single exposure setup. \textbf{(d)}, \textbf{(e)}, and \textbf{(f)}: raw change in attitudes, aggregated across participants, mid- (after 7 sessions) and post-intervention (after 14 sessions) in the longitudinal exposure setup. Across all 3 DVs and the single, longitudinal exposure setups, the change in participants' attitudes, post intervention, enrolled in the LLM intervention was higher (and hence, more approving) compared to that for participants enrolled in the Human intervention (e.g., $0.178$ vs. $-0.060$ after a single exposure for DV3 -- (c)). For participants in the LLM condition, the change in attitudes was more pronounced, in the less stigmatizing direction, after a longitudinal exposure compared to a single exposure intervention -- e.g., $0.412$ vs. $0.178$ for DV3 ((f) vs. (c)). Interventions were the most effective in reducing stigmatizing attitudes toward MAT, i.e., DV3 -- e.g., for the single exposure intervention (LLM) change in attitudes were $-0.135$, $-0.019$, and $0.178$ ((a) vs. (b) vs. (c)).}
\label{fig:raw_change}
\end{figure*}

==> figures/figure4-scatter-plots-control.tex <==
\begin{figure*}
\centering
    \begin{subfigure}[b]{0.33\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/single-shot_scatter_control_DV1.pdf}
    \caption{} \label{fig:single-shot_scatter_control_DV1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.33\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/single-shot_scatter_control_DV2.pdf}
    \caption{} \label{fig:single-shot_scatter_control_DV2}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.33\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/single-shot_scatter_control_DV3.pdf}
    \caption{} \label{fig:single-shot_scatter_control_DV3}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.33\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/repeated-exp_scatter_control_DV1.pdf}
    \caption{} \label{fig:repeated-exp_scatter_control_DV1}
    \end{subfigure}
    \begin{subfigure}[b]{0.33\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/repeated-exp_scatter_control_DV2.pdf}
    \caption{} \label{fig:repeated-exp_scatter_control_DV2}
    \end{subfigure}
    \begin{subfigure}[b]{0.33\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/repeated-exp_scatter_control_DV3.pdf}
    \caption{} \label{fig:repeated-exp_scatter_control_DV3}
    \end{subfigure}
    \caption{}
\label{fig:scatter-plots-control}
\end{figure*}
